Do we expect to find the Super-Earths close to the gas giants?

We have investigated the evolution of a pair of interacting planets embedded in a gaseous disc, considering the possibility of the resonant capture of a Super-Earth by a Jupiter mass gas giant. First, we have examined the situation where the Super-Earth is on the internal orbit and the gas giant on the external one. It has been found that the terrestrial planet is scattered from the disc or the gas giant captures the Super-Earth into an interior 3:2 or 4:3 mean-motion resonance. The stability of the latter configurations depends on the initial planet positions and on eccentricity evolution. The behaviour of the system is different if the Super-Earth is the external planet. We have found that instead of being captured in the mean-motion resonance, the terrestrial planet is trapped at the outer edge of the gap opened by the gas giant. This effect prevents the occurrence of the first order mean-motion commensurability. These results are particularly interesting in light of recent exoplanet discoveries and provide predictions of what will become observationally testable in the near future.

==> R_E_A_D_M_E <==

List of files, besides the original contribution, with an explanation.
-----------------------------------------------------------------------

* ms.edit.pdf - PDF file with the final text (after editorial changes).

  Language and format changes are marked in red.
  Queries to the Author/s and Referee's comments are marked 
  in blue at the right-hand margin.

* ms.edit.tex - the source file with the language and format corrections.

  Changes are marked by \langeditorchanges{}; longer fragments through:

  \newcommand\langeditorstart{ }  
  \newcommand\langeditorstop{ }  

  and \edchange{}

  Referee's/editorial notes are marked by \ednote{}.

  Definitions of these macros are included in the the text 
  through an external file editor.tex, see the source text's preamble, 
  as follows:

  %%HIGHLIGHT_CHANGES_BEGIN
  \input editor.tex
  %%HIGHLIGHT_CHANGES_END

  To get rid of the markup, please comment out the following lines
  at the end of the editor.tex file:

  %
  %\renewcommand\langeditorchanges[1]{#1}
  %\renewcommand\langeditorstart{}
  %\renewcommand\langeditorstop{}
  %\renewcommand\edchange[1]{}
  %\renewcommand\ednote[1]{}
  %
    
* ms.orig.tex  - a copy of the contributed text in the original form.

* ms.highlight.tex - the source file with language correction only,
  which might be useful to see the differences with the ms.orig.tex
  (e.g., via the Unix' "diff" command).

* eps2pdf a scropt that converts .eps/.ps figures to .pdf format with
  the help of epstopdf utility.

The source file should be converted directly to PDF format through 

pdflatex ms.edit.tex 

which produces the "ms.edit.pdf"

Please note that figures ".eps" and ".ps" files have been converted to 
.pdf format.

In some cases, the psfig macro-commands might have been changed
\includegraphics{} command from "the graphicx" package.

---
Krzysztof Gozdziewski
k.gozdziewski@astri.umk.pl



